A New Upper Bound on the Maximal Error Resilience of Interactive Error-Correcting Codes

In an interactive error-correcting code (iECC), Alice and Bob engage in an interactive protocol with the goal of Alice communicating a message $x \in \{ 0, 1 \}^k$ to Bob in such a way that even if some fraction of the total communicated bits are corrupted, Bob can still determine $x$. It was shown in works by Gupta, Kalai, and Zhang (STOC 2022) and by Efremenko, Kol, Saxena, and Zhang (FOCS 2022) that there exist iECCs that are resilient to a larger fraction of errors than is possible in standard error-correcting codes without interaction. One major question in the study of iECCs is to determine the optimal error resilience achievable by an iECC. In the case of bit flip errors, it is known that an iECC can achieve $\frac14 + 10^{-5}$ error resilience (Efremenko, Kol, Saxena, and Zhang), while the best known upper bound is $\frac27 \approx 0.2857$ (Gupta, Kalai, and Zhang). In this work, we improve upon the upper bound, showing that no iECC can be resilient to more than $\frac{13}{47} \approx 0.2766$ fraction of errors.

==> lemmas.tex <==
\section{Helpful Lemmas}

We begin with a series of helpful lemmas that make it easier to describe the adversary's attacks.

% \begin{lemma} \label{lem:dist-14-strings} \rnote{not useful? / reproved in below lemma}
%     Given three strings $s_1, s_2, s_3 \in \{ 0, 1 \}^\ell$ such that $\Delta (s_x, s_y) \le \left( \frac12 + \epsilon \right) \cdot \ell$ for all $x \not= y \in \{ 1, 2, 3 \}$, there exists string $t \in \{ 0, 1 \}^\ell$ such that 
%     \[
%         \Delta(t, s_x) \le \left( \frac14 + \frac\epsilon2 \right) \cdot \ell ~~\forall x \in \{ 1, 2, 3 \}.
%     \]
% \end{lemma}

% \begin{proof}
%     Let $I_{123}$ be the indices for which $s_1[i] = s_2[i] = s_3[i]$, and let $I_{12}$, $I_{23}$, and $I_{31}$ be the indices $\subseteq [\ell]$ for which $s_1[i] = s_2[i] \not= s_3[i]$, $s_2[i] = s_3[i] \not= s_1[i]$, and $s_3[i] = s_1[i] \not= s_2[i]$, respectively. Notice that $I_{123} \cup I_{12} \cup I_{23} \cup I_{31} = [\ell]$. 

%     We define the string $t$ as follows. For all indices $i \in I_{123}$, we define $t[i] := s_1[i] = s_2[i] = s_3[i]$. For each $I_{xy}$, if $|I_{xy}| \le \left( \frac14 + \frac\epsilon2 \right) \cdot \ell$, we define $t[i] := s_x[i] = s_y[i]$. Otherwise, if $|I_{xy}| > \left( \frac14 + \frac\epsilon2 \right) \cdot \ell$, we define $t[i] := s_x[i] = s_y[i]$ for $\left( \frac14 + \frac\epsilon2 \right) \cdot \ell$ indices $i \in I_{xy}$, and for the rest of the indicies $i \in I_{xy}$, we define $t[i] := 1 - s_x[i] = 1 - s_y[i]$.

%     Now, note that since $\Delta(s_x, s_y) \le \left( \frac12 + \epsilon \right) \cdot \ell$ for all $x \not= y \in [3]$, it holds that at most one of $I_{12}$, $I_{23}$, and $I_{31}$ can have more than $\left( \frac14 + \frac\epsilon2 \right) \cdot \ell$ elements (if for instance $|I_{12}|, |I_{23}| > \left( \frac14 + \frac\epsilon2 \right) \cdot \ell$, then $\Delta(s_1, s_3) > \left( \frac12 + \epsilon \right) \cdot \ell$). If all of $I_{12}, I_{23}, I_{31}$ have size at most $\left( \frac14 + \frac\epsilon2 \right) \cdot \ell$, then 
%     \[
%         \Delta(t, s_x) = |I_{yz}| \le \left( \frac14 + \frac\epsilon2 \right) \cdot \ell,
%     \]
%     where $y, z \in [3]$ are the other two indices not equal to $x$. Otherwise, exactly one of $I_{12}, I_{23}, I_{31}$ has size greater than $\left( \frac14 + \frac\epsilon2 \right) \cdot \ell$. Without loss of generality suppose that $|I_{12}| > \left( \frac14 + \frac\epsilon2 \right) \cdot \ell$. Then, 
%     \begin{align*}
%         \Delta(t, s_1) &= |I_{23}| + |I_{12}| - \left( \frac14 + \frac\epsilon2 \right) \cdot \ell \le \left( \frac12 + \epsilon \right) \cdot \ell - \left( \frac14 + \frac\epsilon2 \right) \cdot \ell = \left( \frac14 + \frac\epsilon2 \right) \cdot \ell \\
%         \Delta(t, s_2) &= |I_{13}| + |I_{12}| - \left( \frac14 + \frac\epsilon2 \right) \cdot \ell \le \left( \frac12 + \epsilon \right) \cdot \ell - \left( \frac14 + \frac\epsilon2 \right) \cdot \ell = \left( \frac14 + \frac\epsilon2 \right) \cdot \ell \\
%         \Delta(t, s_3) &= \left( \frac14 + \frac\epsilon2 \right) \cdot \ell.
%     \end{align*}
% \end{proof}





